What Does the Virial Coefficient of the \Hb Broad-Line Region Depend On?

We combine our dynamical modeling black hole mass measurements from the Lick AGN Monitoring Project 2016 sample with measured cross-correlation time lags and line widths to recover individual scale factors, f, used in traditional reverberation mapping analyses. We extend our sample by including prior results from Code for AGN Reverberation and Modeling of Emission Lines (caramel) studies that have utilized our methods. Aiming to improve the precision of black hole mass estimates, as well as uncover any regularities in the behavior of the broad-line region (BLR), we search for correlations between f and other AGN/BLR parameters. We find (i) evidence for a correlation between the virial coefficient log10(fmean,{\sigma}) and black hole mass, (ii) marginal evidence for a similar correlation between log10(frms,{\sigma}) and black hole mass, (iii) marginal evidence for an anti-correlation of BLR disk thickness with log10(fmean,FWHM)and log10(frms,FWHM), and (iv) marginal evidence for an anti-correlation of inclination angle with log10(fmean,FWHM), log10(frms,{\sigma}), and log10(fmean,{\sigma}). Lastly, we find marginal evidence for a correlation between line-profile shape, when using the root-meansquare spectrum, log10(FWHM/{\sigma})rms, and the virial coefficient, log10(frms,{\sigma}), and investigate how BLR properties might be related to line-profile shape using caramel models.

==> line_profile_param_linear_regression.tex <==
\begin{deluxetable*}{c l c cccccc}
\tablecaption{Linear regression results for line profile shape}
\tablewidth{0pt}
\setlength{\tabcolsep}{8pt}
\tablehead{
\colhead{Line Profile Shape} &
\colhead{ } &
\colhead{$\log_{10}(M_{\rm bh}/M_{\odot})$ } &
\colhead{$\theta_i$ (${\rm deg.}$)} &
\colhead{$\theta_o$ (${\rm deg.}$)} &
\colhead{$\log_{10}(L_{\rm bol}/L_{\rm Edd})$ } 
}
\startdata
\multirow{ 3}{*}{\begin{tabular}{l} $\log_{10}\Big(\frac{\rm{FWHM}}{\sigma}\Big)_{\rm{mean}}$ \\ \end{tabular}} % & $\alpha$ & 7.18$^{+ 0.22} _{- 0.22}$  & 25.12$^{+ 4.35} _{- 4.35}$ & 27.96$^{+ 5.73} _{- 5.73}$ & -0.7$^{+ 0.23} _{- 0.23}$ \\
 & $\alpha$ & -0.03$^{+ 0.38} _{- 0.38}$  & 0.33$^{+ 0.12} _{- 0.12}$ & 0.25$^{+ 0.09} _{- 0.09}$ & 0.1$^{+ 0.05} _{- 0.05}$ \\
% & $\beta$ & 0.4$^{+ 0.69} _{- 0.69}$ & -2.74$^{+ 13.81} _{- 13.81}$ & 3.39$^{+ 18.06} _{- 18.06}$ & -1.93$^{+ 0.73} _{- 0.73}$  \\
& $\beta$ & 0.04$^{+ 0.05} _{- 0.05}$ & -0.0$^{+ 0.01} _{- 0.01}$ & 0.0$^{+ 0.01} _{- 0.01}$ & -0.15$^{+ 0.04} _{- 0.04}$  \\
% & $\sigma_{\rm int}$ & 0.23$^{+ 0.09} _{- 0.09}$  & 56.34$^{+ 35.07} _{- 35.07}$ & 109.01$^{+ 53.56} _{- 53.56}$& 0.25$^{+ 0.1} _{- 0.1}$  \\ \hline 
& $\sigma_{\rm int}$ & 0.15$^{+ 0.0} _{- 0.0}$ & 0.15$^{+ 0.0} _{- 0.0}$ & 0.15$^{+ 0.0} _{- 0.0}$& 0.13$^{+ 0.0} _{- 0.0}$   \\ \hline 
 \multirow{ 3}{*}{\begin{tabular}{l} $\log_{10}\Big(\frac{\rm{FWHM}}{\sigma}\Big)_{\rm{rms}}$ \\ \end{tabular}}  
 %& $\alpha$ & 7.02$^{+ 0.24} _{- 0.24}$ &  28.78$^{+ 5.27} _{- 5.27}$ & 29.19$^{+ 6.6} _{- 6.6}$ &  -0.76$^{+ 0.26} _{- 0.26}$ \\
  & $\alpha$ & -0.55$^{+ 0.57} _{- 0.57}$ & 0.46$^{+ 0.22} _{- 0.22}$ & 0.27$^{+ 0.15} _{- 0.15}$ & 0.11$^{+ 0.09} _{- 0.09}$ \\
 %& $\beta$ & 1.2$^{+ 0.79} _{- 0.79}$  & -16.15$^{+ 18.06} _{- 18.06}$  &  1.2$^{+ 0.79} _{- 0.79}$ & -1.82$^{+ 0.86} _{- 0.86}$  \\
  & $\beta$ & 0.11$^{+ 0.08} _{- 0.08}$   & -0.01$^{+ 0.01} _{- 0.01}$  &  0.0$^{+ 0.01} _{- 0.01}$ & -0.13$^{+ 0.06} _{- 0.06}$  \\
% & $\sigma_{\rm int}$ &  0.21$^{+ 0.09} _{- 0.09}$ &  56.66$^{+ 42.55} _{- 42.55}$ & 111.78$^{+ 61.44} _{- 61.44}$ &  0.25$^{+ 0.12} _{- 0.12}$  \\ 
  & $\sigma_{\rm int}$ &  0.14$^{+ 0.01} _{- 0.01}$ &  0.14$^{+ 0.01} _{- 0.01}$ &  0.15$^{+ 0.01} _{- 0.01}$ &  0.13$^{+ 0.01} _{- 0.01}$ \\ 
\enddata
\tablecomments{Linear regression results for line profile shape vs. BLR/AGN parameters using both the mean and rms spectrum. $\alpha$ represents the constant in the regression and $\beta$ represents the slope of the regression, while $\sigma_{\rm{int}}^2$ represents the variance of the intrinsic scatter. The corresponding relationship is therefore given by $\log_{10}(\rm{FWHM/}\sigma)= \alpha + \beta\times \rm{parameter}+\mathcal{N}(0,\sigma_{\rm int})$.}
\label{tab:lineprofile_params_linear_regression}
\end{deluxetable*}

==> line_profile_shape_nocovariance.tex <==
\begin{deluxetable}{c l c cccccc}
\tablecaption{Linear regression results (no covariance) for \\ line profile shape vs. scale factor}
%\tablewidth{0pt}
\setlength{\tabcolsep}{6pt}
\tablehead{
\colhead{Line Profile Shape} &
\colhead{ } &
\colhead{$\log_{10}f_{\sigma}$} &
\colhead{$\log_{10}f_{\rm{FWHM}}$}
}
\startdata
\multirow{ 3}{*}{\begin{tabular}{l} $\log_{10}\Big(\frac{\rm{FWHM}}{\sigma}\Big)_{\rm{mean}}$ \\ \end{tabular}}  & $\alpha$ &
0.34$^\pm 0.16$ & 0.33$\pm 0.16$ \\
%&  0.34$^{+ 0.14} _{- 0.14}$ &  0.34$^{+ 0.14} _{- 0.14}$ \\
 & $\beta$ & 0.84$^\pm 0.50$ &$-1.2\pm 0.5$ \\
%0.73$^{+ 0.44} _{- 0.45}$ &  $-1.26^{+ 0.45} _{- 0.45}$  \\
 & $\sigma_{\rm int}$ & 0.39$^{+ 0.07} _{- 0.05}$ & 0.39$^{+ 0.07} _{- 0.05}$ \\ \hline
 %0.26$^{+ 0.05} _{- 0.05}$  &  0.26$^{+ 0.05} _{- 0.05}$  \\ \hline
 \multirow{ 3}{*}{\begin{tabular}{l} $\log_{10}\Big(\frac{\rm{FWHM}}{\sigma}\Big)_{\rm{rms}}$ \\ \end{tabular}}  & $\alpha$ & 0.44$\pm 0.19$ & 0.44$^{+ 0.22} _{- 0.23}$ \\
 %0.37$^{+ 0.19} _{- 0.19}$ & 0.38$^{+ 0.23} _{- 0.23}$  \\
 & $\beta$  &  0.81$^{+ 0.62} _{- 0.61}$ & $-1.12^{+ 0.70} _{- 0.69}$ \\
 %0.96$^{+ 0.63} _{- 0.63}$ &  $-1.08^{+ 0.76} _{- 0.76}$   \\
 & $\sigma_{\rm int}$  &  0.43$^{+ 0.08} _{- 0.06}$  &  0.46$^{+ 0.10} _{- 0.07}$ \\
 %0.30$^{+ 0.07} _{- 0.07}$ &  0.35$^{+ 0.10} _{- 0.10}$
\enddata
\tablecomments{Linear regression results for line profile shape vs. scale factor. The parameters $\alpha$ and $\beta$ represent the constant and slope of the regression, respectively, while $\sigma_{\rm{int}}$ represents the standard deviation of the intrinsic scatter. The corresponding relationship is therefore given by $\log_{10}(\rm{FWHM/}\sigma)= \alpha + \beta \log_{10}(\textit{f})+\mathcal{N}(0,\sigma_{\rm int})$.}
\label{tab:mean_lineprofile_f_linear_regression}
\end{deluxetable}

==> meanf.tex <==
\newcommand{\combinedmeanfrmssigma}{$0.65\pm0.07$}%{$0.62 \pm 0.07$}
\newcommand{\combinedsigmafrmssigma}{$0.22\pm0.09$}%{$0.23 \pm 0.09$}
\newcommand{\combinedpredfrmssigma}{$0.65\pm 0.25$}%{$0.62 \pm 0.26$}

\newcommand{\combinedmeanfrmsfwhm}{$0.16\pm 0.08$}%{$0.15 \pm 0.08$}
\newcommand{\combinedsigmafrmsfwhm}{$0.30\pm0.08$}%{$0.30\pm 0.08$}
\newcommand{\combinedpredfrmsfwhm }{$0.16\pm0.32$}%{$0.15 \pm 0.32$}

\newcommand{\combinedmeanfmeansigma}{$0.56\pm0.07$}%{$0.54 \pm 0.07$}
\newcommand{\combinedsigmafmeansigma}{$0.25\pm0.08$}%{$0.25 \pm 0.08$}
\newcommand{\combinedpredfmeansigma}{$0.56\pm0.27$}
%{$0.54 \pm 0.27$}

\newcommand{\combinedmeanfmeanfwhm}{$0.02\pm 0.08$}
%{$0.02 \pm 0.08$}
\newcommand{\combinedsigmafmeanfwhm}{$0.32\pm 0.08$}
%{$0.32 \pm 0.08$}
\newcommand{\combinedpredfmeanfwhm}{$0.02\pm 0.34$}%{$0.02 \pm 0.34$}

%\newcommand{\combinedmeanfrmsfwhm}{$0.57 \pm 0.07$}
%\newcommand{\combinedsigmafrmsfwhm}{$0.14 \pm 0.10$}
%\newcommand{\combinedpredfrmsfwhm}{$0.57 \pm 0.19$}

\newcommand{\lampmeanfrmssigma}{$0.85\pm 0.13$}
%{$0.18 \pm 0.15$}
%{$0.79\pm 0.17$}
\newcommand{\lampsigmafrmssigma}{$0.24\pm 0.17$}
%{$0.26 \pm 0.17$}
%{$0.33 \pm 0.18$}
\newcommand{\lamppredfrmssigma}{$0.85\pm 0.31$}
%{$0.85 \pm 0.34$}
%{$0.79 \pm 0.41$}


\newcommand{\lampmeanfmeansigma}{$0.76\pm0.13$}%{$0.69 \pm 0.16$}
\newcommand{\lampsigmafmeansigma}{$0.23\pm 0.16$}%{$0.31 \pm 0.17$}
\newcommand{\lamppredfmeansigma}{$0.76\pm 0.31$}%{$0.68 \pm 0.39$}

\newcommand{\lampmeanfmeanfwhm}{$0.02\pm0.12$}
%{$-0.04\pm0.11$}
\newcommand{\lampsigmafmeanfwhm}{$0.19\pm0.13$}%{$0.20 \pm 0.11$}
\newcommand{\lamppredfmeanfwhm}{$0.02\pm 0.26$}%{$-0.04 \pm 0.26$}

\newcommand{\lampmeanfrmsfwhm}{$0.18\pm0.13$}
%{$0.14 \pm 0.12$}
\newcommand{\lampsigmafrmsfwhm}{$0.22\pm 0.14$}
%{$0.21 \pm 0.13$}
\newcommand{\lamppredfrmsfwhm}{$0.18 \pm 0.29$}%{$0.14 \pm 0.27$}



==> table_meanf.tex <==
\input{meanf}
\begin{deluxetable*}{c l c c c c}
\tablecaption{Summary of Scale Factors}
\setlength{\tabcolsep}{14pt}
%\tablewidth{1.8pt}
\tablehead{
\colhead{ } &
\colhead{ } &
\colhead{mean, FWHM} &
\colhead{mean, $\sigma$} &
\colhead{rms, $\sigma$} &
\colhead{rms, FWHM}
}
\startdata
 & $\langle \log_{10}{f}\rangle$ & \lampmeanfmeanfwhm & \lampmeanfmeansigma & \lampmeanfrmssigma  & \lampmeanfrmsfwhm \\
L16 & $\sigma_{\langle \log_{10}f\rangle}$ & \lampsigmafmeanfwhm & \lampsigmafmeansigma & \lampsigmafrmssigma & \lampsigmafrmsfwhm  \\
 & $\langle \log_{10}f \rangle _{\rm pred}$ & \lamppredfmeanfwhm & \lamppredfmeansigma & \lamppredfrmssigma &  \lamppredfrmsfwhm \\\hline
 & $\langle \log_{10} f \rangle$ & \combinedmeanfmeanfwhm & \combinedmeanfmeansigma & \combinedmeanfrmssigma & \combinedmeanfrmsfwhm \\
Comb. & $\sigma_{\langle \log_{10}f \rangle }$ & \combinedsigmafmeanfwhm & \combinedsigmafmeansigma & \combinedsigmafrmssigma & \combinedsigmafrmsfwhm \\
 & $\langle \log_{10}f \rangle _{\rm pred}$ & \combinedpredfmeanfwhm & \combinedpredfmeansigma & \combinedpredfrmssigma & \combinedpredfrmsfwhm \\
\enddata
\tablecomments{Summary of the scale factors calculated for the LAMP 2016 sample \citepalias{Villafa_a_2022} and Combined \citetalias{Villafa_a_2022} + \citetalias{2018ApJ...866...75W} + \citetalias{Grier++17} + \citetalias{pancoast14b} + \citetalias{2020ApJ...902...74W} + \citetalias{bentz2021detailed} + B22 sample (Comb.). The mean scale factor is $\langle \log_{10}{f} \rangle$, the dispersion is $\sigma_{\langle \log_{10}f \rangle}$, and the mean and standard deviation of the posterior predictive distribution is $\langle \log_{10}f \rangle _{\rm pred}$. These values are found to be consistent with values found in the literature, within their uncertainties. }
\label{tab:table_meanf}
\end{deluxetable*}
